INT v.s. FP: A Comprehensive Study of Fine-Grained Low-bit Quantization Formats

Modern AI hardware, such as Nvidia's Blackwell architecture, is increasingly embracing low-precision floating-point (FP) formats to handle the pervasive activation outliers in Large Language Models (LLMs). Despite this industry trend, a unified comparison of FP and integer (INT) quantization across varying granularities has been missing, leaving algorithm and hardware co-design without clear guidance. This paper fills that gap by systematically investigating the trade-offs between FP and INT formats. We reveal a critical performance crossover: while FP excels in coarse-grained quantization, the comparison at fine-grained (block-wise) levels is more nuanced. Our comprehensive comparison demonstrates that for popular 8-bit fine-grained formats (e.g., MX with block size 32), MXINT8 is superior to its FP counterpart in both algorithmic accuracy and hardware efficiency. However, for 4-bit formats, FP (e.g., MXFP4, NVFP4) often holds an accuracy advantage , though we show that NVINT4 can surpass NVFP4 when outlier-mitigation techniques like Hadamard rotation are applied. We also introduce a symmetric clipping method that resolves gradient bias in fine-grained low-bit INT training, enabling nearly lossless performance for MXINT8 training. These findings challenge the current hardware trajectory, demonstrating that a one-size-fits-all FP approach is suboptimal and advocating that fine-grained INT formats, particularly MXINT8, offer a better balance of accuracy, power, and efficiency for future AI accelerators.

==> figure_tex/compute_flow.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.4\linewidth]{figures/quant_flow.pdf}
    \caption{Compute flow of low-bit forward and backward probation of linear layer.}
    \label{fig:quant_flow}
\end{figure}

==> figure_tex/hardware_cost_vs_bs.tex <==
\begin{figure}[!h]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/hardware/sweep_block_size.pdf}
    \caption{Normalized area and energy cost vs. block size for FP8/4 and INT8/4 formats.}
    \begin{minipage}{\linewidth}
    \footnotesize
    \begin{itemize}
    \item For INT8: Block size $=1$ $\Rightarrow$ \texttt{BF16} behavior
    \item For INT8: Block size $\to \infty$ $\Rightarrow$ native \texttt{INT8} behavior
    \end{itemize}
    \end{minipage}
    \label{fig: sweep_block_size}
\end{figure}


==> figure_tex/inference_kl.tex <==
\begin{figure}[!t]
    \centering
    \begin{subfigure}[b]{0.45\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/inference_kl.pdf}
        \caption{Direct-cast inference.}
        \label{fig:inference_kl_a}
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.45\linewidth}
        \centering
\includegraphics[width=\linewidth]{figures/inference_kl_rotation.pdf}
        \caption{Direct-cast inference(w/ Hadamard rotation).}
        \label{fig:inference_kl_b}
    \end{subfigure}
    \caption{INT v.s. FP on 12 models through KL divergence on WikiText2. (a) shows the results with direct-cast inference, while (b) shows the results with direct-cast inference combined with random Hadamard rotation. Detailed numbers can be found in Sec.~\ref{sec:detailed_results}.}
    \label{fig:inference_kl}
\end{figure}

==> figure_tex/int_range_ablation.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{figures/int_range_ablation.pdf}
    \caption{Impact of clipping range on INT8 final training loss on 145M model with 20B training tokens. Scale factor is kept on BF16 to emphasize the harm of asymmetric representation space during training.}
    \label{fig:int_range_ablation}
\end{figure}

==> figure_tex/kappa_boxplot.tex <==
\begin{figure}[!t]
    \centering
    \begin{subfigure}[b]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/crest_factor_box_1x3.pdf}
        \caption{Crest factor}\label{fig:crest_factor}
    \end{subfigure}
    \begin{subfigure}[b]{0.48\linewidth}
        \centering
\includegraphics[width=\linewidth]{figures/crest_factor_box_1x3_rotate.pdf}
        \caption{Crest factor w/ hadamard rotation}\label{fig:crest_factor_rotation}
    \end{subfigure}
    \caption{Boxplots of crest factor across different block size, outliers are plotted as points. ``-1'' indicates channel-wise quantization granularities. Detailed numbers of boxplots can be find in Table~\ref{tab:crest_factor}.}\label{fig:crest_factor}
    \label{fig:crest_factor_all}
\end{figure}

==> figure_tex/mixed_format.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{figures/normalized_area_vs_dtype.pdf}
    \caption{The area cost of MMU under different low-bit formats specifications. The throughput ratio of 8-bit to 4-bit is set to 1:2 to match the communication bandwidth.}
    \label{fig:area_vs_dtype}
\end{figure}

==> figure_tex/qsnr.tex <==
\begin{figure}[!t]
    \centering
\includegraphics[width=0.9\linewidth]{figures/qsnr_int_fp_8_6_4_combined_top_legend.pdf}
    \caption{QSNR versus block size for quantization across 6 forward/backward items. -1 denotes per-channel quantization. 8-bit and 6-bit use E8M0 scales for MX-format, and 4-bit uses E4M3 scales for NV-format. Detailed numbers can be find in Table.~\ref{tab:qsnr}.}
    \label{fig:qsnr}
\end{figure}

==> figure_tex/qsnr_rotation.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{figures/qsnr_rotation.pdf}
    \caption{QSNR versus block size for quantization of \textcircled{1} $\mathbf{X}$ with random Hadamard Rotation. Numbers after the arrow indicates the QSNR gain brought by using rotation at block size 16.  Detailed numbers can be find in Table.~\ref{tab:qsnr_rotation}.}
    \label{fig:qsnr_rotation}
\end{figure}

==> figure_tex/theoretical_comparions.tex <==
\begin{figure}[!t]
    \centering
    \begin{subfigure}[b]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/qsnr_vs_kappa.pdf}
        \caption{QSNR comparisons across crest factor $\kappa$.}
        \label{fig:qsnr_vs_kappa}
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.48\linewidth}
        \centering
\includegraphics[width=\linewidth]{figures/crest_factor.pdf}
        \caption{Crest factor decrease with smaller block size.}
        \label{fig:crest_factor}
    \end{subfigure}
    \caption{ \textbf{Theoretical analysis of quantization performance.} (a) QSNR comparison between various integer (INT) and floating-point (FP) formats across a range of crest factors ($\kappa$), derived from Eq.~(\ref{eq:int_qsnr}) and Eq.~(\ref{eq:fp_qsnr}). The boxes represent the crest factor and QSNR of the intersection point of the INT and FP curves. (b) The effect of quantization block size on the average crest factor for a gaussian distribution and an outlier-prone distribution from Llama-3.1-8B activations. }
    \label{fig:theory}
\end{figure}

==> sections/A_hardware_model_bk.tex <==


\input{tables/hardware/gate_complexity}

\section{Hardware Cost Modeling}~\label{sec:hardware_model_cost}
% \begin{figure}[!h]
%     \centering
%     \includegraphics[width=0.7\linewidth]{figures/hardware/microarchitecture diagram.pdf}
%     \caption{Microarchitecture diagram of hardware implementation.}
%     \label{fig: microarchitecture diagram}
% \end{figure}
\paragraph{Scope and assumptions.}
We develop a compact gate-level model to estimate the chip area and energy of a GEMM engine under low-precision formats. Specifically, a low-bit GEMM engine uses four components: a quantizer, a multiply-and-accumulate (MAC) unit, a dequantizer, and an FP32 accumulator. The proposed model accounts only for the MAC unit, a shared FP32 accumulator and a dequantizer; the quantizer is excluded from all cost accounting. In MX/NV formats, the VPU implements quantization by shift/divide-and-round, and the accumulation pipeline can fuse dequantization as two 8-bit integer additions for UE8M0 scale or two floating-point multiplications for E4M3 scale. We omit the quantizer block in VPU to isolate the cost driven by multiplication and accumulation. Unless otherwise stated, we take cell factors from a TSMC FinFET standard-cell library. We model only combinational logic; we ignore sequential elements, placement and routing, and interconnect to enable technology-aware, relative comparisons.

\paragraph{Design choice: FP32 accumulation and MMU integration.}
A high-throughput Matrix-Multiply Unit (MMU), as in TPU-like designs~\citep{tpu}, integrates the multiply-and-accumulate datapath and downstream accumulation to improve performance and energy efficiency. To prevent error growth and preserve scalability, we accumulate in FP32. Under the same nominal bit width, FP multipliers are typically more area- and energy-efficient than INT multipliers, whereas FP adders are more expensive than INT adders due to exponent comparison/subtraction, mantissa alignment, and normalization~\citep{fp_vs_int}. With a uniform-alignment design~\cite{fp_adders}, the normalizer count reduces to one shared instance across the $k$ MAC lanes, and we divide its cost by $k$.

\paragraph{Mantissa aligner width.}
The mantissa aligner couples accuracy and cost: its bit width $n$ affects numerical fidelity and hardware complexity. We set
\begin{equation}
\label{eq: aligner_width}
	n \;=\; \min\!\bigl(2^{x+1} + 2y,\; \texttt{psum\_bit\_width}\bigr),
\end{equation}
where $x$ and $y$ denote exponent and mantissa widths, respectively (for INT formats, $x\!=\!0$). In all evaluations we use $k\!=\!32$ and $\texttt{psum\_bit\_width}\!=\!24$.

\paragraph{MAC unit structure and sub-blocks.}
We model the MAC unit as a $k$-lane array. Each lane comprises one multiplier. The adders from all lanes are fused together to form a multi-input adder tree structure, incorporating FP-specific alignment and normalization logic. Table~\ref{tab: mac_complexity} reports the dominant logic count (up to constant factors) for the main sub-blocks, where ``Main Cells'' indicate the standard-cell types used for area/energy aggregation. For FP multiplication, we multiply only mantissas and include an exponent adder. For FP addition, we model exponent comparator/subtractor, a barrel aligner, a wide mantissa adder, and one shared normalizer. For INT, we set $x\!=\!0$ in the expressions.

\paragraph{Area and energy aggregation for MAC.}
Let $\mathcal{S}$=\{Multiplier, Adder(mantissa/int), Exponent adder, Exponent subtractor, Comparator, Aligner(barrel), Normalizer(shared)\} be the set of sub-block types,
and $\mathcal{G}=\{\text{FA},\text{HA},\text{XOR},\text{AND},\text{OR},\text{MUX}\}$ be the set of cell types with technology-dependent area and energy factors $A_g$ and $E_g$ obtained from the standard-cell library. Let $\tau_g$ be the toggle rate of cell $g$, which represents the average switching activity of the cell. In this work, we simplify the toggle rate factor by assuming that all gate cells have the same toggle rate, $\tau_g=\tau$, to reduce computational complexity and focus on the primary design trade-offs. Denote by $c_{s,g}(x,y,k,n)$ the count of cell $g\in\mathcal{G}$ in sub-block $s$ induced by the chosen format and by $n$ from Eq.(\ref{eq: aligner_width}). The MAC area and energy are
\begin{equation}
\text{Area}_{\text{MAC}} \;=\; \sum_{s\in\mathcal{S}}\sum_{g\in\mathcal{G}} c_{s,g}(x,y,k,n)\,A_g,\qquad
\text{Energy}_{\text{MAC}} \;=\; \sum_{s\in\mathcal{S}}\sum_{g\in\mathcal{G}} c_{s,g}(x,y,k,n)\,E_g \tau_g.
\end{equation}

\paragraph{FP32 accumulator model.}
We model the FP32 accumulator by its combinational logic counts $c^{\text{ACC32}}_{g}$, yielding
\begin{equation}
\text{Area}_{\text{ACC32}} \;=\; \sum_{g\in\mathcal{G}} c^{\text{ACC32}}_{g}\,A_g,\qquad
\text{Energy}_{\text{ACC32}} \;=\; \sum_{g\in\mathcal{G}} c^{\text{ACC32}}_{g}\,E_g.
\end{equation}

\paragraph{Total cost and per-lane reporting.}
The total MMU cost is
\begin{equation}
\text{Area}_{\text{MMU}} \;=\; \text{Area}_{\text{MAC}} + \text{Area}_{\text{ACC32}},\qquad
\text{Energy}_{\text{MMU}} \;=\; \text{Energy}_{\text{MAC}} + \text{Energy}_{\text{ACC32}},
\end{equation}
and, when we report per-lane figures, we divide the cost of shared blocks by $k$.

% \input{figure_tex/hardware_cost_vs_bs}

\paragraph{Summary.}
The hardware model includes only the MAC unit and the FP32 accumulator; the quantizer and dequantizer are excluded from the overhead calculation. Given a low-precision format with exponent/mantissa widths $(x,y)$ (with $x{=}0$ for INT), a MAC array size $k$, an aligner cap $\texttt{psum\_bit\_width}$ (setting $n$ via Eq~(\ref{eq: aligner_width}), and technology cell factors $\{A_g,E_g\}_{g\in\mathcal{G}}$ (plus the FP32-accumulator gate counts), the model predicts the area and energy of the MAC and accumulation stages. It captures the relative cost trends across INT/FP/MX formats at the same nominal bit width, the sensitivity to the aligner width $n$ (critical for FP addition), and the effect of sharing both the normalizer and the FP32 accumulator across $k$ lanes.




==> sections/Abstract.tex <==
\begin{abstract}
Modern AI hardware, such as Nvidia's Blackwell architecture, is increasingly embracing low-precision floating-point (FP) formats to handle the pervasive activation outliers in Large Language Models (LLMs). Despite this industry trend, a unified comparison of FP and integer (INT) quantization across varying granularities has been missing, leaving algorithm and hardware co-design without clear guidance. This paper fills that gap by systematically investigating the trade-offs between FP and INT formats. We reveal a critical performance crossover: while FP excels in coarse-grained quantization, INT consistently surpasses it as the quantization block size shrinks. Our comprehensive comparison demonstrates that for popular fine-grained formats like MX (block size 32), MXINT8 and MXINT4 are superior to their FP counterparts in both algorithmic accuracy and hardware efficiency. We also introduce a symmetric clipping method that resolves gradient bias in fine-grained low-bit INT training, enabling nearly lossless performance for MXINT8 training. These findings challenge the current hardware trajectory and advocate for prioritizing fine-grained INT formats in future AI accelerators to achieve a better balance of accuracy, power, and efficiency.



%Despite this industry trend, a comprehensive comparison between FP and integer (INT) quantization across varying group sizes under a unified framework is conspicuously absent, leaving future algorithm and hardware design without clear guidance. This paper systematically investigates this issue and reveals a critical performance crossover point: while FP formats excel in coarse-grained quantization, INT formats consistently surpass them as the quantization granularity becomes finer. We provide the first comprehensive comparison of these formats across a spectrum of granularities, demonstrating that for the popular MX format (block size=32), MXINT8 and MXINT4 is superior to MXFP8 and MXFP4 in both algorithmic accuracy and hardware efficiency.  Furthermore, we propose a symmetric clipping method to resolve the gradient bias problem in fine-grained INT quantization-aware training. Our findings challenge the current hardware design trajectory and strongly suggest that future AI accelerators should prioritize INT formats with fine-grained quantization to achieve a superior balance of accuracy and power efficiency.
\end{abstract}

==> sections/distribution_analysis.tex <==
\section{Distribution Analysis: The "Why" Behind Quantization Challenges.}

% LLM has significant outlier in forward activation, such as regular channel-wise outliers and non-regular massive activation caused by swiglu mechanism.    

\subsection{Methodology}

\subsection{Distribution Visualization and Insights}




==> sections/fp4_vs_int4.tex <==
\section{Pushing the Limits: An Exploration of 4-Bit Quantization}
\subsection{Head-to-Head: MXINT4 vs. MXFP4}

\subsection{Future-Facing: The Synergy of INT4 and Rotation}


==> sections/fp8_vs_int8.tex <==
\section{FP8 vs. INT8}


\subsection{Methodology}
This paper try to give a comprehensive comparisons of integer quantization and float-point quantization across different quantization granularities. In particular, we construct a multi-scale evaluation paradigm to evaluate the quantization error in a local-to-global manner. Specifically, this evaluation pipeline includes three settings:
\begin{itemize}
    \item Layer-wise quantization error. Figure~\ref{fig:quant_flow} shows that there are 2 quantization operation and 4 quantization operation for forward and backward of GEMM, respectively. We 
    \item End-to-end inference quantization error.
    \item End-to-end training quantization error.
\end{itemize}

\begin{itemize}
    \item Layer-wise QSNR. Following~\citep{qsnr}, we use Quantization Signal to Noise Ratio~(QSNR) as a measure of numerical fidelity under different quantization schemes. QSNR is defined as the ratio of the power of the non-quantized signal to the 
power of the quantization noise expressed in decibels. It is calculated as:
 \begin{equation}  \label{eq:qsnr_def}
 \resizebox{0.6\linewidth}{!}{$ 
\begin{aligned}
\text{QSNR} &:= -10 \, \text{log} (\frac{\mathbb{E}[\lVert Q(\mathbf{X}) - \mathbf{X} \rVert^{2}]}{\mathbb{E}[\lVert \mathbf{X} \rVert^{2}]}),
\end{aligned}$}
\end{equation}
where $\lVert \mathbf{X} \rVert := (\sum_{i=1}^{k}{x_{i}^{2}})^{1/2}$, and $Q(\cdot)$ is the quantization function which maps $k$-dimensional 
arrays with FP32 precision to the target quantization format. A higher QSNR indicates that the 
quantized vector better preserves the direction and magnitude of the original non-quantized vector in the space $\mathbb{R}^{k}$.
    \item End-to-End inference.
    \item End-to-end training.
\end{itemize}





\textbf{Inference}

\textbf{Training}

\textbf{Comparisons}

\subsection{Experiments Results}

\subsubsection{Layer-wise Analysis}
\input{tables/qsnr/qsnr_fp8}
\input{tables/qsnr/qsnr_int8}
% figure in main paper
% table in appendix

\textbf{Setups}

\subsubsection{End-to-End Inference}
\input{tables/inference/kl_template}
\textbf{Setups}

\subsubsection{End-to-End  Training}
\input{tables/training/loss_temp}
\input{tables/training/loss_8bit_in_house}a

\textbf{Setups}

==> tables/ablation/e8m0_ablation_qwen.tex <==
\begin{table}[]
\centering
\begin{tabular}{ccc}
\hline
Qtype  & Eq.(\ref{eq:ocp_e8m0})             & Eq.(\ref{eq:our_e8m0})    \\
% Qtype  & OCP (Eq.(\ref{eq:ocp_e8m0}))             & Ours   (Eq.(\ref{eq:our_e8m0})    \\
\hline
BF16 & \multicolumn{2}{c}{6.5135} \\
MXINT8 & 6.519           & \textbf{6.5174} \\
MXFP8  & 6.5655          & \textbf{6.5453} \\
MXINT6 & \textbf{6.6475} & 6.6499          \\
MXFP6  & 6.5795          & \textbf{6.5787} \\
MXINT4 & \textbf{9.0716} & 10.0423         \\
MXFP4  & \textbf{8.8178} & 9.6005  \\ 
\hline
\end{tabular}
\caption{Ablation experiments about UE8M0 scale factors. The Qwen-3-8B perplexity (lower is better) on Wikitext2 with 4096 context length is reported.}
\label{tab:abl_e8m0}
\end{table}

==> tables/ablation/round_e8m0.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{ccccc}
    \hline
    & \multirow{2}{*}{BF16} & \multicolumn{3}{c}{UE8M0} \\
    \cmidrule(l{2pt}r{2pt}){3-5} 
    & & floor & round & ceil \\
    \hline
per-channel & 6.8853 & 9.6893    & 7.0436 & 7.095  \\
256         & 6.5308 & 61.9582   & 6.9358 & 6.5546 \\
128         & 6.5263 & 394.7787  & 7.0264 & 6.5419 \\
64          & 6.5209 & 1899.269  & 7.1134 & 6.5265 \\
32          & 6.5168 & 3971.1343 & 7.1754 & 6.5174 \\
    \hline
    \end{tabular}
    \caption{Ablation experiments about rounding operation in INT8 quantization.}
    \label{tab:abl_round_e8m0}
\end{table}

==> tables/hardware/area_and_energy.tex <==
\begin{table}[!h]
\centering
\caption{Normalized energy and area cost of different low-bit formats at the same throughput.}
\label{tab: cost_comp_single_format}
\begin{tabular}{ccccccc}
\hline
                        & MXFP8        & MXINT8       & MXFP6        & MXINT6       & MXFP4        & MXINT4 \\ \hline
\begin{tabular}[c]{@{}c@{}}Normalized\\ Energy\end{tabular}       & $\times1.00$ & $\times0.67$ & $\times0.53$ & $\times0.41$ & $\times0.31$ & $\times0.23$   \\ \hline
\begin{tabular}[c]{@{}c@{}}Normalized\\ Area\end{tabular}         & $\times1.00$ & $\times0.83$ & $\times0.53$ & $\times0.50$ & $\times0.29$ & $\times0.27$  \\ \hline
% Element Type            & E4M3         & INT8(E0M7)   & E2M3         & INT6(E0M5)   & E2M1         & INT4(E0M3)   \\ \hline
% Block Size              & \multicolumn{6}{c}{32}                                          \\ \hline
% Scale Type              & \multicolumn{6}{c}{UE8M0}                                       \\ 
% \hline
\end{tabular}

\end{table}

==> tables/hardware/area_and_energy_2_backup.tex <==
\begin{table}[!h]
\centering
\caption{Normalized energy and area costs of low-bit formats at same throughput. Single-format results use MXFP8 as the baseline, and mixed-format results use MXFP8+NVFP4 as the baseline.}
\label{tab:energy_area}
\setlength{\tabcolsep}{3pt}
\begin{tabular}{ccccccc|cc}
\hline
        & \multicolumn{6}{c}{Single Format} & \multicolumn{2}{c}{Mixed Format} \\
        \hline
        & MXFP8  & MXINT8  & MXFP4 & MXINT4 & NVFP4 & NVINT4 & MXFP8+NVFP4     & MXINT8+NVINT4     \\
         \hline
Energy & 1x     & \textbf{0.63x}  & 0.41x & \textbf{0.22x}  & 0.55x   & \textbf{0.34x}   & 1x              &    \textbf{0.75x}         \\
\hline
Area   & 1x     & \textbf{0.79x}  & 0.40x & \textbf{0.25x}  & 0.54x   & \textbf{0.38x}   & 1x              &    \textbf{0.66x}         \\
\hline
\end{tabular}
\end{table}

==> tables/inference/kl_template.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{lccccc}
    \hline
    & per-channel & 256 & 128 & 64 & 32 \\
    \hline 
    \textcircled{1} $\mathbf{X}$ & & & & & \\
    \hline 
    \textcircled{2} $\mathbf{W}$ & & & & & \\
    \hline
    \textcircled{1} $\mathbf{X}$ +  \textcircled{2} $\mathbf{W}$  & & & & & \\
    \hline
    \end{tabular}
    \caption{KL divergence of *** quantization across different quantization settings and quantization granularities on *** Model.}
    \label{tab:kl_temp}
\end{table}

==> tables/qsnr/qsnr.tex <==
\begin{table}[!h]
\centering
\caption{QSNR versus block size for quantization across 6 types of forward/backward items. -1 denotes per-channel quantization. E4M3 scales contains another FP32 per-tensor scale factor just like NV-format.}
\label{tab:qsnr}
\begin{tabular}{cclcccccc}
\hline
Format                & Scales Type           & Item                                            & G = -1 & 256   & 128   & 64    & 32    & 16    \\
\hline
\multirow{6}{*}{INT8} & \multirow{6}{*}{E8M0} & \textcircled{1} $\mathbf{X}$   & 27.55  & 33.73 & 35.41 & 37.20 & 38.96 & 40.74 \\
                      &                       & \textcircled{2} $\mathbf{W}$   & 36.81  & 38.97 & 39.72 & 40.59 & 41.51 & 42.47 \\
                      &                       & \textcircled{3} $\mathbf{dY}$  & 29.00  & 35.02 & 36.60 & 37.87 & 39.30 & 40.50 \\
                      &                       & \textcircled{4} $\mathbf{W}^T$ & 36.00  & 38.69 & 39.56 & 40.42 & 41.45 & 42.44 \\
                      &                       & \textcircled{5} $\mathbf{X}^T$ & 36.46  & 38.71 & 39.59 & 40.54 & 41.56 & 42.65 \\
                      &                       & \textcircled{6} $\mathbf{dY}$  & 25.12  & 31.09 & 33.11 & 35.08 & 37.04 & 38.85 \\
\cdashline{1-9}
\multirow{6}{*}{FP8}  & \multirow{6}{*}{E8M0} & \textcircled{1} $\mathbf{X}$   & 31.21  & 31.23 & 31.23 & 31.23 & 31.23 & 31.23 \\
                      &                       & \textcircled{2} $\mathbf{W}$   & 31.27  & 31.27 & 31.27 & 31.27 & 31.27 & 31.27 \\
                      &                       & \textcircled{3} $\mathbf{dY}$  & 31.22  & 31.23 & 31.23 & 31.23 & 31.23 & 31.22 \\
                      &                       & \textcircled{4} $\mathbf{W}^T$ & 31.27  & 31.27 & 31.27 & 31.27 & 31.27 & 31.27 \\
                      &                       & \textcircled{5} $\mathbf{X}^T$ & 31.23  & 31.23 & 31.23 & 31.23 & 31.23 & 31.23 \\
                      &                       & \textcircled{6} $\mathbf{dY}$  & 31.22  & 31.22 & 31.22 & 31.22 & 31.22 & 31.22 \\
                      \hline
\multirow{6}{*}{INT6} & \multirow{6}{*}{E8M0} & \textcircled{1} $\mathbf{X}$   & 15.69  & 21.66 & 23.33 & 25.15 & 26.96 & 28.82 \\
                      &                       & \textcircled{2} $\mathbf{W}$   & 24.68  & 26.91 & 27.68 & 28.58 & 29.60 & 30.70 \\
                      &                       & \textcircled{3} $\mathbf{dY}$  & 17.84  & 23.30 & 24.82 & 26.19 & 27.83 & 29.41 \\
                      &                       & \textcircled{4} $\mathbf{W}^T$ & 23.87  & 26.62 & 27.51 & 28.41 & 29.53 & 30.66 \\
                      &                       & \textcircled{5} $\mathbf{X}^T$ & 24.52  & 26.74 & 27.62 & 28.61 & 29.69 & 30.87 \\
                      &                       & \textcircled{6} $\mathbf{dY}$  & 15.68  & 20.95 & 22.82 & 24.70 & 26.70 & 28.74 \\
                      \cdashline{1-9}
\multirow{6}{*}{FP6}  & \multirow{6}{*}{E8M0} & \textcircled{1} $\mathbf{X}$   & 20.78  & 26.02 & 27.22 & 28.33 & 29.21 & 29.89 \\
                      &                       & \textcircled{2} $\mathbf{W}$   & 28.42  & 29.58 & 29.84 & 30.10 & 30.34 & 30.55 \\
                      &                       & \textcircled{3} $\mathbf{dY}$  & 22.20  & 27.02 & 28.05 & 28.81 & 29.55 & 30.08 \\
                      &                       & \textcircled{4} $\mathbf{W}^T$ & 27.89  & 29.43 & 29.77 & 30.04 & 30.32 & 30.54 \\
                      &                       & \textcircled{5} $\mathbf{X}^T$ & 27.91  & 29.20 & 29.59 & 29.95 & 30.26 & 30.52 \\
                      &                       & \textcircled{6} $\mathbf{dY}$  & 19.60  & 24.63 & 26.15 & 27.49 & 28.65 & 29.54 \\
                      \hline
\multirow{6}{*}{INT4} & \multirow{6}{*}{E4M3} & \textcircled{1} $\mathbf{X}$   & 7.33   & 12.52 & 14.13 & 15.91 & 17.70 & 19.59 \\
                      &                       & \textcircled{2} $\mathbf{W}$   & 14.71  & 17.41 & 18.19 & 19.03 & 19.98 & 21.12 \\
                      &                       & \textcircled{3} $\mathbf{dY}$  & 9.72   & 14.11 & 15.40 & 16.74 & 18.33 & 19.98 \\
                      &                       & \textcircled{4} $\mathbf{W}^T$ & 14.01  & 17.08 & 17.99 & 18.84 & 19.91 & 21.08 \\
                      &                       & \textcircled{5} $\mathbf{X}^T$ & 15.26  & 17.42 & 18.27 & 19.21 & 20.28 & 21.51 \\
                      &                       & \textcircled{6} $\mathbf{dY}$  & 9.56   & 13.73 & 15.33 & 16.96 & 18.76 & 20.69 \\
                      \cdashline{1-9}
\multirow{6}{*}{FP4}  & \multirow{6}{*}{E4M3} & \textcircled{1} $\mathbf{X}$   & 9.88   & 14.17 & 15.32 & 16.53 & 17.70 & 18.96 \\
                      &                       & \textcircled{2} $\mathbf{W}$   & 15.33  & 16.60 & 16.94 & 17.33 & 17.85 & 18.58 \\
                      &                       & \textcircled{3} $\mathbf{dY}$  & 11.43  & 15.00 & 15.85 & 16.76 & 17.79 & 18.94 \\
                      &                       & \textcircled{4} $\mathbf{W}^T$ & 14.89  & 16.47 & 16.87 & 17.29 & 17.84 & 18.58 \\
                      &                       & \textcircled{5} $\mathbf{X}^T$ & 15.42  & 16.53 & 16.93 & 17.38 & 17.93 & 18.64 \\
                      &                       & \textcircled{6} $\mathbf{dY}$  & 11.43  & 15.42 & 16.80 & 18.17 & 19.62 & 21.19 \\
                      \hline
\multirow{6}{*}{INT4} & \multirow{6}{*}{E8M0} & \textcircled{1} $\mathbf{X}$   & 5.25   & 9.71  & 11.18 & 12.85 & 14.53 & 16.29 \\
                      &                       & \textcircled{2} $\mathbf{W}$   & 11.86  & 14.18 & 14.82 & 15.60 & 16.57 & 17.70 \\
                      &                       & \textcircled{3} $\mathbf{dY}$  & 7.57   & 11.46 & 12.64 & 13.90 & 15.41 & 16.96 \\
                      &                       & \textcircled{4} $\mathbf{W}^T$ & 11.28  & 13.85 & 14.65 & 15.44 & 16.50 & 17.66 \\
                      &                       & \textcircled{5} $\mathbf{X}^T$ & 12.29  & 14.24 & 15.02 & 15.92 & 16.93 & 18.07 \\
                      &                       & \textcircled{6} $\mathbf{dY}$  & 8.11   & 11.72 & 13.12 & 14.55 & 16.11 & 17.77 \\
                      \cdashline{1-9}
\multirow{6}{*}{FP4}  & \multirow{6}{*}{E8M0} & \textcircled{1} $\mathbf{X}$   & 7.62   & 11.86 & 12.99 & 14.13 & 15.11 & 15.94 \\
                      &                       & \textcircled{2} $\mathbf{W}$   & 13.11  & 15.13 & 15.48 & 15.82 & 16.17 & 16.55 \\
                      &                       & \textcircled{3} $\mathbf{dY}$  & 9.65   & 13.11 & 13.94 & 14.73 & 15.55 & 16.21 \\
                      &                       & \textcircled{4} $\mathbf{W}^T$ & 12.74  & 14.90 & 15.36 & 15.73 & 16.14 & 16.54 \\
                      &                       & \textcircled{5} $\mathbf{X}^T$ & 13.55  & 14.96 & 15.41 & 15.86 & 16.29 & 16.69 \\
                      &                       & \textcircled{6} $\mathbf{dY}$  & 9.55   & 12.72 & 13.74 & 14.66 & 15.51 & 16.22 \\
                      \hline
\end{tabular}
\end{table}

==> tables/qsnr/qsnr_rotation.tex <==
\begin{table}[!h]
\centering
\caption{QSNR versus block size \textbf{with random Hadamard rotation} for quantization across 6 types of forward/backward items. -1 denotes per-channel quantization. E4M3 scales contains another FP32 per-tensor scale factor just like NV-format.}
\label{tab:qsnr_rotation}
\begin{tabular}{cclcccccc}
\hline
Format                & Scale Type           & Item                                            & G = -1                    & 256                       & 128                       & 64                        & 32                        & 16                        \\
\hline
\multirow{6}{*}{INT8} & \multirow{6}{*}{E8M0} & \textcircled{1} $\mathbf{X}$   & 35.07                     & 39.32                     & 40.30                     & 41.24                     & 42.27                     & 43.06                     \\
                      &                       & \textcircled{2} $\mathbf{W}$   & 37.95                     & 39.46                     & 40.12                     & 40.89                     & 41.75                     & 42.63                     \\
                      &                       & \textcircled{3} $\mathbf{dY}$  & 34.55                     & 39.02                     & 40.27                     & 41.07                     & 42.01                     & 42.47                     \\
                      &                       & \textcircled{4} $\mathbf{W}^T$ & 37.56                     & 39.23                     & 39.99                     & 40.76                     & 41.74                     & 42.63                     \\
                      &                       & \textcircled{5} $\mathbf{X}^T$ & 36.76                     & 39.05                     & 39.92                     & 40.83                     & 41.82                     & 42.66                     \\
                      &                       & \textcircled{6} $\mathbf{dY}$  & 32.94                     & 38.63                     & 40.39                     & 42.03                     & 43.51                     & 43.67                     \\
                      \cdashline{1-9}
\multirow{6}{*}{FP8}  & \multirow{6}{*}{E8M0} & \textcircled{1} $\mathbf{X}$   & 31.26                     & 31.26                     & 31.26                     & 31.26                     & 31.26                     & 31.26                     \\
                      &                       & \textcircled{2} $\mathbf{W}$   & 31.25                     & 31.25                     & 31.25                     & 31.25                     & 31.25                     & 31.25                     \\
                      &                       & \textcircled{3} $\mathbf{dY}$  & 31.24                     & 31.24                     & 31.24                     & 31.24                     & 31.24                     & 31.23                     \\
                      &                       & \textcircled{4} $\mathbf{W}^T$ & 31.25                     & 31.25                     & 31.25                     & 31.25                     & 31.25                     & 31.25                     \\
                      &                       & \textcircled{5} $\mathbf{X}^T$ & 31.26                     & 31.26                     & 31.26                     & 31.26                     & 31.26                     & 31.26                     \\
                      &                       & \textcircled{6} $\mathbf{dY}$  & 31.24                     & 31.24                     & 31.24                     & 31.24                     & 31.24                     & 31.24                     \\
                      \hline
\multirow{6}{*}{INT6} & \multirow{6}{*}{E8M0} & \textcircled{1} $\mathbf{X}$   & 22.93                     & 27.24                     & 28.28                     & 29.28                     & 30.40                     & 31.31                     \\
                      &                       & \textcircled{2} $\mathbf{W}$   & 25.86                     & 27.43                     & 28.09                     & 28.91                     & 29.86                     & 30.87                     \\
                      &                       & \textcircled{3} $\mathbf{dY}$  & 22.69                     & 27.10                     & 28.36                     & 29.32                     & 30.55                     & 31.41                     \\
                      &                       & \textcircled{4} $\mathbf{W}^T$ & 25.45                     & 27.20                     & 27.96                     & 28.77                     & 29.85                     & 30.87                     \\
                      &                       & \textcircled{5} $\mathbf{X}^T$ & 24.60                     & 26.94                     & 27.90                     & 28.85                     & 29.90                     & 30.86                     \\
                      &                       & \textcircled{6} $\mathbf{dY}$  & 21.32                     & 26.95                     & 28.80                     & 30.64                     & 32.47                     & 33.03                     \\
                      \cdashline{1-9}
\multirow{6}{*}{FP6}  & \multirow{6}{*}{E8M0} & \textcircled{1} $\mathbf{X}$   & 27.15                     & 29.65                     & 30.03                     & 30.31                     & 30.54                     & 30.67                     \\
                      &                       & \textcircled{2} $\mathbf{W}$   & 29.13                     & 29.80                     & 29.99                     & 30.20                     & 30.40                     & 30.58                     \\
                      &                       & \textcircled{3} $\mathbf{dY}$  & 26.72                     & 29.51                     & 30.02                     & 30.29                     & 30.55                     & 30.67                     \\
                      &                       & \textcircled{4} $\mathbf{W}^T$ & 28.87                     & 29.70                     & 29.95                     & 30.16                     & 30.40                     & 30.58                     \\
                      &                       & \textcircled{5} $\mathbf{X}^T$ & 28.29                     & 29.55                     & 29.87                     & 30.18                     & 30.43                     & 30.60                     \\
                      &                       & \textcircled{6} $\mathbf{dY}$  & 25.66                     & 29.21                     & 29.92                     & 30.43                     & 30.78                     & 30.84                     \\
                      \hline
\multirow{6}{*}{INT4} & \multirow{6}{*}{E4M3} & \textcircled{1} $\mathbf{X}$   & 12.64                     & 17.12                     & 18.28                     & 19.44                     & 20.65                     & 22.02                     \\
                      &                       & \textcircled{2} $\mathbf{W}$   & 15.72                     & 17.91                     & 18.59                     & 19.33                     & 20.22                     & 21.30                     \\
                      &                       & \textcircled{3} $\mathbf{dY}$  & 12.80                     & 16.99                     & 18.22                     & 19.24                     & 20.54                     & 21.92                     \\
                      &                       & \textcircled{4} $\mathbf{W}^T$ & 15.33                     & 17.60                     & 18.41                     & 19.18                     & 20.18                     & 21.30                     \\
                      &                       & \textcircled{5} $\mathbf{X}^T$ & 14.73                     & 17.11                     & 18.06                     & 19.08                     & 20.19                     & 21.38                     \\
                      &                       & \textcircled{6} $\mathbf{dY}$  & 11.99                     & 16.86                     & 18.55                     & 20.28                     & 22.07                     & 23.92                     \\
                      \cdashline{1-9}
\multirow{6}{*}{FP4}  & \multirow{6}{*}{E4M3} & \textcircled{1} $\mathbf{X}$   & 13.95                     & 16.51                     & 17.00                     & 17.45                     & 17.95                     & 18.56                     \\
                      &                       & \textcircled{2} $\mathbf{W}$   & 15.86                     & 16.77                     & 17.05                     & 17.39                     & 17.87                     & 18.56                     \\
                      &                       & \textcircled{3} $\mathbf{dY}$  & 13.95                     & 16.45                     & 16.96                     & 17.39                     & 17.92                     & 18.56                     \\
                      &                       & \textcircled{4} $\mathbf{W}^T$ & 15.65                     & 16.66                     & 17.00                     & 17.36                     & 17.87                     & 18.56                     \\
                      &                       & \textcircled{5} $\mathbf{X}^T$ & 15.31                     & 16.53                     & 16.93                     & 17.39                     & 17.93                     & 18.62                     \\
                      &                       & \textcircled{6} $\mathbf{dY}$  & 13.77                     & 17.00                     & 17.81                     & 18.49                     & 19.07                     & 19.57                     \\
                      \hline
\multirow{6}{*}{INT4} & \multirow{6}{*}{E8M0} & \textcircled{1} $\mathbf{X}$   & {9.64}  & {13.85} & {14.97} & {16.06} & {17.21} & {18.50} \\
                      &                       & \textcircled{2} $\mathbf{W}$   & {12.89} & {14.65} & {15.20} & {15.89} & {16.80} & {17.88} \\
                      &                       & \textcircled{3} $\mathbf{dY}$  & {10.17} & {14.04} & {15.18} & {16.18} & {17.44} & {18.75} \\
                      &                       & \textcircled{4} $\mathbf{W}^T$ & {12.45} & {14.39} & {15.06} & {15.75} & {16.76} & {17.88} \\
                      &                       & \textcircled{5} $\mathbf{X}^T$ & {11.47} & {13.84} & {14.71} & {15.71} & {16.73} & {17.89} \\
                      &                       & \textcircled{6} $\mathbf{dY}$  & {9.92}  & {14.22} & {15.77} & {17.33} & {18.96} & {20.64} \\
                      \cdashline{1-9}
\multirow{6}{*}{FP4}  & \multirow{6}{*}{E8M0} & \textcircled{1} $\mathbf{X}$   & {11.78} & {14.75} & {15.41} & {15.96} & {16.42} & {16.84} \\
                      &                       & \textcircled{2} $\mathbf{W}$   & {13.74} & {15.40} & {15.69} & {15.97} & {16.28} & {16.63} \\
                      &                       & \textcircled{3} $\mathbf{dY}$  & {12.10} & {14.90} & {15.52} & {15.99} & {16.49} & {16.90} \\
                      &                       & \textcircled{4} $\mathbf{W}^T$ & {13.58} & {15.22} & {15.61} & {15.90} & {16.27} & {16.63} \\
                      &                       & \textcircled{5} $\mathbf{X}^T$ & {13.16} & {14.74} & {15.25} & {15.75} & {16.20} & {16.63} \\
                      &                       & \textcircled{6} $\mathbf{dY}$  & {11.67} & {14.74} & {15.57} & {16.27} & {16.85} & {17.29} \\
                      \hline
\end{tabular}
\end{table}

==> tables/qsnr/qsnr_template.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{lccccc}
    \hline
    & per-channel & 256 & 128 & 64 & 32 \\
    \hline 
    \textcircled{1} $\mathbf{X}$ & & & & & \\
    \hline
    \textcircled{2} $\mathbf{W}$ & & & & & \\
    \hline
    \textcircled{3} $\mathbf{dY}$ & & & & & \\
    \hline
    \textcircled{4} $\mathbf{W}^T$ & & & & & \\
    \hline
    \textcircled{5} $\mathbf{X}^T$ & & & & & \\
    \hline
    \textcircled{6} $\mathbf{dY}$ & & & & & \\
    \hline
    \end{tabular}
    \caption{Average QSNR of *** quantization across different quantized objects and quantization granularities on *** Model.}
    \label{tab:qsnr_temp}
\end{table}

==> tables/training/loss_8bit.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{ccccccc}
    \hline
    Model Size & QType & per-channel & 256 & 128 & 64 & 32 \\
    \hline
    \multirow{2}{*}{M}& FP & \\
    & INT & \\
    \hline
    \multirow{2}{*}{M}& FP & \\
    & INT & \\
    \hline
    \multirow{2}{*}{M}& FP & \\
    & INT & \\
    \hline
    \end{tabular}
    \caption{Caption}
    \label{tab:loss_8bit}
\end{table}

==> tables/training/loss_8bit_in_house.tex <==
% 站内大模型试验结果
\begin{table}[]
    \centering
    \begin{tabular}{cccc}
    \hline
    Model Size & Training Tokens & QType & Final Loss \\
    \hline
    & & BF16 & \\
    & & MXINT8 \\
    \hline
    & & BF16 & \\
    & & MXINT8 \\
    \hline
    & & BF16 & \\
    & & MXINT8 \\
    \hline
    \end{tabular}
    \caption{MXINT8 training of in-house models. [TODO] add some accuracy results.}
    \label{tab:in_house_MXINT8}
\end{table}

==> tables/training/loss_temp.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{ccccccc}
    \hline
    Model Size & QType & per-channel & 256 & 128 & 64 & 32 \\
    \hline
    \multirow{2}{*}{M}& FP & \\
    & INT & \\
    \hline
    \multirow{2}{*}{M}& FP & \\
    & INT & \\
    \hline
    \multirow{2}{*}{M}& FP & \\
    & INT & \\
    \hline
    \end{tabular}
    \caption{Caption}
    \label{tab:loss_temp}
\end{table}
